Beyond Demographics: Aligning Role-playing LLM-based Agents Using Human Belief Networks

Creating human-like large language model (LLM) agents is crucial for faithful social simulation. Having LLMs role-play based on demographic information sometimes improves human likeness but often does not. This study assessed whether LLM alignment with human behavior can be improved by integrating information from empirically-derived human belief networks. Using data from a human survey, we estimated a belief network encompassing 64 topics loading on nine non-overlapping latent factors. We then seeded LLM-based agents with an opinion on one topic, and assessed the alignment of its expressed opinions on remaining test topics with corresponding human data. Role-playing based on demographic information alone did not align LLM and human opinions, but seeding the agent with a single belief greatly improved alignment for topics related in the belief network, and not for topics outside the network. These results suggest a novel path for human-LLM belief alignment in work seeking to simulate and understand patterns of belief distributions in society.

==> figures/FA_loading_matrix_factor_1_5.tex <==
\begin{figure}[th!] 
\centering
\includegraphics[width=1\linewidth]{figures/FA_loading_matrix_factor_1_5_fig.pdf}
\vspace{-2mm}
\caption{Partial factor loading matrix from the Belief Survey. This matrix includes the columns for these Ghost (\textcolor{green}{\textbf{green}}) and the Partisan (\textcolor{violet}{\textbf{violet})} factors and the rows for topics that belong to these two factor categories (i.e., having the highest loadings on one of these two factors). Red indicates topics that load highly on a factor, gray indicates near 0 loading, and blue indicates loading in the negative direction. The topics in the Ghost category has minimal loading on the Partisan factor and vice versa (highlighted by the black boxes). The training topics are further highlighted by \textcolor{darkgreen}{\textbf{dark green}} and \textcolor{purple}{\textbf{purple}} boxes, respectively. The full statement of the each topic is detailed in Table~\ref{tab:list_topic} (\Scref{app:list_topic}). The full factor loading matrix is in Figure~\ref{fig:fa_loading_matrix} (\Scref{app:full_factor_loading_matrix}). \sn{Consider a ``network'' visualization}}
\label{fig:fa_loading_matrix_factor_1_5}
\vspace{-4mm}
\end{figure}


==> figures/belief_network_and_FA_loading_matrix_factor_1_5.tex <==
\begin{figure*}[th!] 
\centering
\includegraphics[width=1\linewidth]{figures/belief_network_and_FA_loading_matrix_factor_1_5_fig.pdf}
\vspace{-2mm}
\caption{The belief network estimated by factor analysis from human respondents' responses on the Belief Survey. (a) Partial factor loading matrix that includes the columns for these Ghost (\textcolor{green}{\textbf{green}}) and the Partisan (\textcolor{violet}{\textbf{violet})} factors and the rows for topics that belong to these two factor categories. The full factor loading matrix is in Figure~\ref{fig:fa_loading_matrix} (\Scref{app:full_factor_loading_matrix}). Red indicates topics that load positively on a factor, gray indicates near 0 loading, and blue indicates loading in the negative direction. The topics in the Ghost category has minimal loading on the Partisan factor and vice versa (highlighted by the black boxes). The training topics are further highlighted by \textcolor{darkgreen}{\textbf{dark green}} (``Dead Talk'') and \textcolor{purple}{\textbf{purple}} (``Gun Control'') boxes, respectively. The full statement of the each topic is in Table~\ref{tab:list_topic} (\Scref{app:list_topic}). (b) The graphical respresentation of the belief network, where the central nodes are the two latent factors, and the leaves (rectangles) are the individual topics. \textcolor{darkred}{Red} and \textcolor{darkblue}{\textbf{blue}} edges indicate positive and negative loadings, respectively. The width of each edge encodes the strength of the loading. The training topics are highlighted with grey backgrounds.}
\label{fig:fa_loading_matrix_factor_1_5}
% \vspace{-4mm}
\end{figure*}


==> tables/result_factor_chatgpt.tex <==
\begin{table}[tbhp!]
\centering
\LARGE
% \small
% \resizebox{0.7\linewidth}{!}{    
\resizebox{1\linewidth}{!}{    
  \begin{tabular}{@{}llcccccc@{}} 
    \toprule
    \multirow{2}{*}{Category} & \multirow{2}{*}{Topic} & \multicolumn{5}{c}{Condition for LLM Agent Construction} \\ 
    \cmidrule(l){3-7} 
    & & None & Demo & Demo+Train & Demo+Train & Demo+Train \\
    & & & & [Diff. Cat.] & [Same Cat.] &  + Query \\
    \cmidrule(r{4pt}){2-6} \cmidrule(l{4pt}){7-7}    
    Ghost & & & & &  \\    
    \hspace{1em} Train & Dead Talk & 0.04 & 0.02 & 0.04 & 0.98 & 1.00 \\
    \cmidrule(r{4pt}){2-6} \cmidrule(l{4pt}){7-7}    
    \hspace{1em} Test & Ghost & 0.03 & 0.05 & -0.07 & \textbf{0.53} & 0.75 \\
    & Alien Visit & -0.08 & -0.05 & -0.04 & \textbf{0.33} & 0.63 \\
    & Soul Walk & -0.05 & 0.06 & -0.07 & \textbf{0.40} & 0.89 \\
    & See Future & -0.03 & 0.07 & -0.03 & \textbf{0.34} & 0.80 \\
    & Astrology & -0.04 & 0.06 & -0.07 & \textbf{0.28} & 0.88 \\
    & Roswell & -0.10 & -0.07 & 0.03 & \textbf{0.26} & 0.85 \\
    & Past Life & -0.02 & 0.01 & 0.09 & \textbf{0.31} & 0.79 \\
    & The Secret & -0.01 & 0.05 & 0.02 &\textbf{0.32} & 0.66 \\
    & Aura & 0.03 & 0.02 & -0.02 & \textbf{0.25} & 0.80 \\
    & Luck & -0.04 & 0.08 & -0.09 & \textbf{0.23} & 0.84 \\
    & Dousing & -0.02 & 0.03 & 0.00 & \textbf{0.19} & 0.71 \\
    \cmidrule(r{4pt}){2-6} \cmidrule(l{4pt}){7-7}    
    Partisan & & & & & & \\
    \hspace{1em} Train & Gun Control & -0.04 & 0.25 & 0.30 & 0.98 & 1.00 \\
    \cmidrule(r{4pt}){2-6} \cmidrule(l{4pt}){7-7}    
    \hspace{1em} Test & Globe Warm & -0.09 & 0.27 & 0.27 & \textbf{0.27} & 0.94 \\
    & Globe Human & -0.10 & 0.30 & 0.35 & \textbf{0.35} & 0.98 \\
    & US Deficit & 0.03 & 0.02 & 0.03 & \textbf{0.16} & 0.70 \\
    & Unions & 0.03 & 0.18 & 0.08 & \textbf{0.18} & 0.88 \\
    & Death Penalty & -0.14 & 0.00 & 0.00 & 0.00 & 0.32 \\
    \bottomrule
  \end{tabular}
}      
\caption{Kendall's Tau coefficients between human respondents and corresponding LLM agents (powered by ChatGPT) for each topic across various LLM agent construction conditions. In particular, the inclusion of within-cluster training topic opinions significantly increases the alignment between human and LLM agent responses within the same cluster. (``Diff. Cat.'' : Different Topic Category; ``Same Cat.'': Same Topic Category) \sn{TODO: Add category-wise metric}}
\label{tab:result_llm_vs_human_chatgpt}
\end{table}


==> tables/result_factor_mistral.tex <==
\begin{table}[tbhp!]
\centering
\LARGE
% \small
\resizebox{1\linewidth}{!}{    
  \begin{tabular}{@{}llcccccc@{}} 
    \toprule
    \multirow{2}{*}{Category} & \multirow{2}{*}{Topic} & \multicolumn{5}{c}{Condition for LLM Agent Construction} \\ 
    \cmidrule(l){3-7} 
    & & None & Demo & Demo+Train & Demo+Train & Demo+Train \\
    & & & & [Diff. Cat.] & [Same Cat.] &  + Query \\
    % \midrule
    \cmidrule(r{4pt}){2-6} \cmidrule(l{4pt}){7-7}    
    Ghost & & & & &  \\    
    \hspace{1em} Train & Dead Talk & NA & NA & 0.07 & 0.97 & 0.98 \\
    % \cmidrule(l){2-7} 
    \cmidrule(r{4pt}){2-6} \cmidrule(l{4pt}){7-7}    
    \hspace{1em} Test & Ghost & NA & NA & NA & \textbf{0.59} & 0.73 \\
    & Alien Visit & NA & NA & NA & \textbf{0.37} & 0.62 \\
    & Soul Walk & NA & NA & 0.07 & \textbf{0.53} & 0.63 \\
    & See Future & NA & NA & -0.08 & \textbf{0.38} & 0.85 \\
    & Astrology & NA & NA & NA & \textbf{0.32} & 0.71 \\
    & Roswell & NA & NA & NA & \textbf{0.21} & 0.28 \\
    & Past Life & NA & NA & -0.05 & \textbf{0.17} & 0.61 \\
    & The Secret & NA & NA & NA & \textbf{0.07} & 0.67 \\
    & Aura & NA & NA & NA & \textbf{0.35} & 0.62 \\
    & Luck & NA & NA & NA & NA & 0.46 \\
    & Dousing & NA & NA & 0.01 & \textbf{0.23} & 0.58 \\
    % \midrule    
    \cmidrule(r{4pt}){2-6} \cmidrule(l{4pt}){7-7}    
    Partisan & & & & & & \\
    \hspace{1em} Train & Gun Control & NA & 0.33 & 0.12 & 0.90 & 0.90 \\
    % \cmidrule(l){2-7}
    \cmidrule(r{4pt}){2-6} \cmidrule(l{4pt}){7-7}    
    \hspace{1em} Test & Globe Warm & NA & 0.32 & 0.22 & \textbf{0.38} & 0.81 \\
    & Globe Human & NA & 0.31 & 0.33 & \textbf{0.39} & 0.73 \\
    & US Deficit & NA & NA & -0.02 & \textbf{0.09} & 0.70 \\
    & Unions & NA & 0.06 & 0.04 & \textbf{0.13} & 0.78 \\
    & Death Penalty & NA & NA & NA & NA & 0.46 \\
    \bottomrule
  \end{tabular}
}      
\caption{Kendall's Tau coefficients between human respondents and corresponding LLM agents (powered by Mistral) for each topic across various LLM agent construction conditions. In particular, the inclusion of within-cluster training topic opinions significantly increases the alignment between human and LLM agent responses within the same cluster. (``Diff. Cat.'' : Different Topic Category; ``Same Cat.'': Same Topic Category) \sn{TODO: Add category-wise metric}}
% \sn{Consider adding the augmented training topic condition to this table.}
\label{tab:result_llm_vs_human_mistral}
\end{table}


% \begin{table}[tbhp!]
% \centering
% \LARGE
% % \small
% \resizebox{1\linewidth}{!}{    
%   \begin{tabular}{@{}llcccccc@{}} 
%     \toprule
%     \multirow{2}{*}{Category} & \multirow{2}{*}{Topic} & \multicolumn{5}{c}{Condition for LLM Agent Construction} \\ 
%     \cmidrule(l){3-7} 
%     & & None & Demo & Demo+Train & Demo+Train & Demo+Train \\
%     & & & & [Diff. Cat.] & [Same Cat.] &  + Query \\
%     % \midrule
%     \cmidrule(r{4pt}){2-6} \cmidrule(l{4pt}){7-7}    
%     Ghost & & & & &  \\    
%     \hspace{1em} Train & Dead Talk & NA & NA & NA & 0.98 & 0.98 \\
%     % \cmidrule(l){2-7} 
%     \cmidrule(r{4pt}){2-6} \cmidrule(l{4pt}){7-7}    
%     \hspace{1em} Test & Ghost & NA & NA & -0.03 & \textbf{0.59} & 0.84 \\
%     & Alien Visit & NA & NA & NA & \textbf{0.36} & 0.74 \\
%     & Soul Walk & NA & NA & NA & \textbf{0.53} & 0.73 \\
%     & See Future & NA & NA & -0.08 & \textbf{0.34} & 0.85 \\
%     & Astrology & NA & NA & NA & \textbf{0.32} & 0.64 \\
%     & Roswell & NA & NA & NA & \textbf{0.28} & 0.50 \\
%     & Past Life & NA & NA & -0.05 & \textbf{0.05} & 0.26 \\
%     & The Secret & NA & NA & NA & \textbf{0.17} & 0.74 \\
%     & Aura & NA & NA & NA & \textbf{0.30} & 0.70 \\
%     & Luck & NA & NA & NA & NA & 0.58 \\
%     & Dousing & NA & NA & 0.06 & \textbf{0.28} & 0.68 \\
%     % \midrule    
%     \cmidrule(r{4pt}){2-6} \cmidrule(l{4pt}){7-7}    
%     Partisan & & & & & & \\
%     \hspace{1em} Train & Gun Control & NA & 0.33 & 0.12 & 0.90 & 0.90 \\
%     % \cmidrule(l){2-7}
%     \cmidrule(r{4pt}){2-6} \cmidrule(l{4pt}){7-7}    
%     \hspace{1em} Test & Globe Warm & NA & 0.32 & 0.22 & \textbf{0.38} & 0.81 \\
%     & Globe Human & NA & 0.31 & 0.33 & \textbf{0.39} & 0.73 \\
%     & US Deficit & NA & NA & -0.02 & \textbf{0.09} & 0.70 \\
%     & Unions & NA & 0.06 & 0.04 & \textbf{0.13} & 0.78 \\
%     & Death Penalty & NA & NA & NA & NA & 0.46 \\
%     \bottomrule
%   \end{tabular}
% }      
% \caption{Kendall's Tau coefficients between human respondents and corresponding LLM agents (powered by Mistral) for each topic across various LLM agent construction conditions. In particular, the inclusion of within-cluster training topic opinions significantly increases the alignment between human and LLM agent responses within the same cluster. (``Diff. Cat.'' : Different Topic Category; ``Same Cat.'': Same Topic Category)}
% % \sn{Consider adding the augmented training topic condition to this table.}
% \label{tab:result_llm_vs_human_mistral}
% \end{table}



==> tables/result_table_merged_chatgpt_mistral.tex <==
\begin{table*}[tbhp!]
\centering
\LARGE
\resizebox{\linewidth}{!}{
  \begin{tabular}{@{}llcccccccccc@{}} 
    \toprule
    \multirow{3}{*}{Category} & \multirow{3}{*}{Topic} & \multicolumn{10}{c}{Conditions for LLM Agent Construction (In-context Learning)} \\ 
    \cmidrule(l){3-12} 
    & & \multicolumn{5}{c}{ChatGPT (\texttt{gpt-3.5-turbo-0125})} & \multicolumn{5}{c}{Mistral (\texttt{Mistral-7B-Instruct-v0.2})} \\
    \cmidrule(r){3-7} \cmidrule(l){8-12}
    & & None & Demo & Demo+Train & Demo+Train & Demo+Train & None & Demo & Demo+Train & Demo+Train & Demo+Train \\
    & & & & [Diff. Cat.] & [Same Cat.] & + Query & & & [Diff. Cat.] & [Same Cat.] & + Query \\
    % \midrule
    \cmidrule(r){1-6} \cmidrule(lr){7-7} \cmidrule(l){8-11} \cmidrule(l){12-12}   
    Ghost & & & & & & & & & & & \\
    \hspace{1em} Train & Dead Talk & 0.04 & 0.02 & 0.04 & 0.98 & 1.00 & NA & NA & 0.07 & 0.97 & 0.98 \\
    \cmidrule(r){2-6} \cmidrule(lr){7-7} \cmidrule(lr){8-11} \cmidrule(l){12-12}        
    \hspace{1em} Test & Ghost & 0.03 & 0.05 & -0.07 & \textbf{0.53} & 0.75 & NA & NA & NA & \textbf{0.59} & 0.73 \\
    & Alien Visit & -0.08 & -0.05 & -0.04 & \textbf{0.33} & 0.63 & NA & NA & NA & \textbf{0.37} & 0.62 \\
    & Soul Walk & -0.05 & 0.06 & -0.07 & \textbf{0.40} & 0.89 & NA & NA & 0.07 & \textbf{0.53} & 0.63 \\
    & See Future & -0.03 & 0.07 & -0.03 & \textbf{0.34} & 0.80 & NA & NA & -0.08 & \textbf{0.38} & 0.85 \\
    & Astrology & -0.04 & 0.06 & -0.07 & \textbf{0.28} & 0.88 & NA & NA & NA & \textbf{0.32} & 0.71 \\
    & Roswell & -0.10 & -0.07 & 0.03 & \textbf{0.26} & 0.85 & NA & NA & NA & \textbf{0.21} & 0.28 \\
    & Past Life & -0.02 & 0.01 & 0.09 & \textbf{0.31} & 0.79 & NA & NA & -0.05 & \textbf{0.17} & 0.61 \\
    & The Secret & -0.01 & 0.05 & 0.02 & \textbf{0.32} & 0.66 & NA & NA & NA & \textbf{0.07} & 0.67 \\
    & Aura & 0.03 & 0.02 & -0.02 & \textbf{0.25} & 0.80 & NA & NA & NA & \textbf{0.35} & 0.62 \\
    & Luck & -0.04 & 0.08 & -0.09 & \textbf{0.23} & 0.84 & NA & NA & NA & NA & 0.46 \\
    & Dousing & -0.02 & 0.03 & 0.00 & \textbf{0.19} & 0.71 & NA & NA & 0.01 & \textbf{0.23} & 0.58 \\
    \cmidrule(r){2-6} \cmidrule(lr){7-7} \cmidrule(lr){8-11} \cmidrule(l){12-12}  
    & $\mae \downarrow$ & [2.42] & [2.54] & [2.31] & \textbf{[1.29]} & [0.34] & [1.82] & [1.82] & [1.83] & \textbf{[1.28]} & [0.71] \\
        
    % \midrule
    \cmidrule(r){1-6} \cmidrule(lr){7-7} \cmidrule(lr){8-11} \cmidrule(l){12-12}
    Partisan & & & & & & & & & & & \\
    \hspace{1em} Train & Gun Control & -0.04 & 0.25 & 0.30 & 0.98 & 1.00 & NA & 0.33 & 0.12 & 0.90 & 0.90 \\
    \cmidrule(r){2-6} \cmidrule(lr){7-7} \cmidrule(lr){8-11} \cmidrule(l){12-12}    
    \hspace{1em} Test & Globe Warm & -0.09 & 0.27 & 0.27 & \textbf{0.27} & 0.94 & NA & 0.32 & 0.22 & \textbf{0.38} & 0.81 \\
    & Globe Human & -0.10 & 0.30 & 0.35 & \textbf{0.35} & 0.98 & NA & 0.31 & 0.33 & \textbf{0.39} & 0.73 \\
    & US Deficit & 0.03 & 0.02 & 0.03 & \textbf{0.16} & 0.70 & NA & NA & -0.02 & \textbf{0.09} & 0.70 \\
    & Unions & 0.03 & 0.18 & 0.08 & \textbf{0.18} & 0.88 & NA & 0.06 & 0.04 & \textbf{0.13} & 0.78 \\
    & Death Penalty & -0.14 & 0.00 & 0.00 & 0.00 & 0.32 & NA & NA & NA & NA & 0.46 \\
    \cmidrule(r){2-6} \cmidrule(lr){7-7} \cmidrule(lr){8-11} \cmidrule(l){12-12}  
    & $ \mae \downarrow$ & [1.42] & [1.32] & [1.35] & \textbf{[1.25]} & [0.38] & [2.20] & [1.32] & [1.39] & \textbf{[1.28]} & [0.63] \\    
    \bottomrule
  \end{tabular}
}      
\caption{Kendall's $\tau_t$ between human respondents and the corresponding LLM agents (powered by ChatGPT and Mistral) for each topic across various LLM agent construction conditions through in-context learning. The bottom row presents the category-wise mean absolute error across the test topics (\mae). The higher the $\tau_t$ and the lower the \mae, the higher the human-LLM alignment. In particular, the inclusion of same-category training topic opinions significantly increases the alignment. (``Diff. Cat.'' : Different Category; ``Same Cat.'': Same Category)}
\label{tab:result_llm_vs_human_chatgpt_mistral}
\end{table*}
